Blockchain-Empowered Trustworthy Data Sharing: Fundamentals, Applications, and Challenges

Various data-sharing platforms have emerged with the growing public demand for open data and legislation mandating certain data to remain open. Most of these platforms remain opaque, leading to many questions about data accuracy, provenance and lineage, privacy implications, consent management, and the lack of fair incentives for data providers. With their transparency, immutability, non-repudiation, and decentralization properties, blockchains could not be more apt to answer these questions and enhance trust in a data-sharing platform. However, blockchains are not good at handling the four Vs of big data (i.e., volume, variety, velocity, and veracity) due to their limited performance, scalability, and high cost. Given many related works proposes blockchain-based trustworthy data-sharing solutions, there is increasing confusion and difficulties in understanding and selecting these technologies and platforms in terms of their sharing mechanisms, sharing services, quality of services, and applications. In this paper, we conduct a comprehensive survey on blockchain-based data-sharing architectures and applications to fill the gap. First, we present the foundations of blockchains and discuss the challenges of current data-sharing techniques. Second, we focus on the convergence of blockchain and data sharing to give a clear picture of this landscape and propose a reference architecture for blockchain-based data sharing. Third, we discuss the industrial applications of blockchain-based data sharing, ranging from healthcare and smart grid to transportation and decarbonization. For each application, we provide lessons learned for the deployment of Blockchain-based data sharing. Finally, we discuss research challenges and open research directions.

==> Tables/Compare_Permissionless_Permissioned.tex <==
\begin{table}[t!]
\caption{\label{tab:table2} Comparisons between permissionless and permissioned blockchain systems.}
\small
\begin{tabularx}{\textwidth}{|l|X|X|}
\hline
\rowcolor{lightgray} \multicolumn{1}{|c|}{\textbf{Properties}}         &  \multicolumn{1}{c}{\textbf{Permissionless systems}}             &  \multicolumn{1}{|c|}{\textbf{Permissioned systems}} \\     
\hline

\textit{Access}  &  Everyone &  Authorized participants \\\hline

\textit{Scope}  &  Large-scale &  Limited	 \\\hline

\textit{Transparency}  &  Transparent &  Vague \\\hline

Data \textit{privacy}  & Poor &  Excellent \\\hline

{\color{red}Participant privacy}  & Anonymous &  Less anonymous \\\hline

\textit{Security}  &  Excellent &  Poor 	 \\\hline

\textit{Scalability}  & Poor & Excellent \\\hline

\textit{Decentralization}  &  Truly decentralized &  Centralized	\\\hline

\textit{Throughput}  &  Low  &  High 	 \\\hline

\textit{Cost}  &  High &  Effective	 \\\hline

\textit{Examples} & Bitcoin \cite{nakamoto2008bitcoin}, Ethereum \cite{buterin2014next, etherplt}& Hyperledger Fabric \cite{androulaki2018hyperledger}, Ripple \cite{schwartz2014ripple} \\
\hline
\end{tabularx}
\end{table}

==> Tables/Compare_PoS_PoW_pBFT.tex <==
\begin{table*}[t!]
\caption{\label{tab:table3} Comparisons among well-known consensus protocols.}
% \small
\centering
\begin{tabular}
{|p{0.23\linewidth}|
 P{0.2\linewidth} | 
 P{0.27\linewidth} | 
 P{0.2\linewidth} |}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{|c|}{\textbf{Properties}} &  \multicolumn{1}{|c|}{\textbf{PoW}}   &  \multicolumn{1}{|c|}{\textbf{PoS}} &  \multicolumn{1}{c|}{\textbf{PBFT}} \\     
\hline

\textit{Finality} & Probabilistic  & Probabilistic \& economic &  Absolute \\
\hline

\textit{Validator/miner selection}  &  Based on hash rate &  Based on stake  & Equal among nodes \\
\hline

\textit{Power consumption} & Very large  &  Negligible & Negligible \\
\hline

\textit{The number of nodes} & Large  &  Medium  &  Small \\\hline

\textit{Fault tolerance} &  < 50\% computing  &  < 50\%  stake & < 33.33\% faulty\\
\hline

\textit{Throughput} &  Low &  High  &  High \\
\hline

\textit{Platforms} & Bitcoin  & PeerCoin, Ethereum 2.0   & Tendermint \\
\hline

\end{tabular}
\end{table*}
